Summary of the 2015 LHCb workshop on multi-body decays of D and B mesons

This document contains a summary of the LHCb workshop on multi-body decays of D and B mesons, held at CBPF, Rio de Janeiro, in July 2015. The workshop was focused on issues related to amplitude analysis of three- and four-body hadronic decays. In addition to selected LHCb results, contributions from guest theorists are included.

==> Stephan-old.tex <==

\subsection{Introduction}
With the advent of large data sets in diffractive production of  exclusive $(3\pi)^{-1}$ ($50-100$ Mevents) it has become possible to extract the structure of the underlying $(2\pi)^0$ isobars ($0^{++}, 1^{--}, 2^{++}, 3^{--}, 4^{++}$) over a wide mass range of the $2\pi$-system using highly developed partial wave analysis tools~\cite{Adolph:2015tqa}.
%\footnote{C. Adolph et al. [COMPASS Collaboration], arXiv:1509.00992 [hep-ex]}.
This extraction is being performed for different values of $J^{PC}$ of
the 3-body system. Although some ambiguities still exist on what
concerns the independent extraction of all isobars in a fully model
independent way, we expect this information to be available soon
\change{(unless hindered by principle issues).}{ (unless we encounter
  unexpected fundamental problems with this approach).}  Thus, not
only \change{}{are} the amplitudes (real and imaginary part) of the
isobaric system \change{is}{} available but one can study their mass
dependence for various values of the angular momentum \change{enclosed
  with}{relative to} the ``spectator'' pion. We expect this
information \change{being}{to provide} valuable input to
\change{describe}{a description of} these systems \change{using a set}{in terms} of universal amplitudes, which could also incorporate
final state interaction (FSI) with the third pion. In addition, one
can vary the momentum of the spectator pion in the isobar rest frame
by varying the mass of the $(3\pi)$-system.

\subsubsection{$J^{PC}$-dependent description of the isobar in a 3-body decay}
\change{COMPASS has shown in a first extraction of the $\pi\pi$ S-wave
  that general features of the $\pi\pi$ S-wave as have been extracted
  from $\pi-\pi$ elastic scattering or a model independent}{A first
  analysis the $\pi\pi$ S-wave in COMPASS data has shown the same
  general features as seen in $\pi\pi$ scattering data or a
  model--independent} analysis of \textrm{$D_s$}-decays~\cite{antimo}
%\footnote{B. Aubert et al. [BaBar collaboration], Phys. Rev. D 79, 032003 (2009)} 
(see LHCb, Belle, Belle II, BaBar, BESIII and others)\change{, can be
reconciled}{}. It is also known from \change{}{the analysis of} $\eta_c$
decays recently presented by the BaBar collaboration (see
hadron2015)~\cite{AntimoPalanoHadron2015}
%\footnote{https://www.jlab.org/conferences/hadron2015/talks/thursday/parallel/session3/\\3C1\_AntimoPalano.pdf},
that the moduli of the $\pi\pi$ amplitudes from various processes vary
considerably, but the mass dependence of the $\pi\pi$ phase shows
little dependence on the system studied (except \change{of}{for} an
overall mass--independent phase factor).  In order to extract
information on more general amplitudes, which may be system
independent, theory \change{}{input} is required to give guidance on
the functional form. \change{$\chi PT$}{Chiral Perturbation Theory
  ($\chi PT$)} allows to calculate\change{d}{} these amplitudes up to
masses of about 400~$MeV/c^2$\change{ and the}{. The} extrapolation to
the threshold for inelastic processes can be performed using
dispersion relations. However, no recipe exists to continue the
$\pi\pi$ amplitude above this mass, nor does it tell us how to include
well known \change{scalar high mass}{high mass scalar} resonances
\change{}{such} as $f_0(1500)$ or above. This information, however, is
crucial for several physics goals:
\begin{itemize} 
\item perform a quasi ``model-independent'' \change{PWA}{Partial Wave
    Analysis (PWA)} of the $(3\pi)^{-1}$ \change{}{system} or even a
  multidimensional PWA, which includes the $(3\pi)^{-1}$ and
  $(2\pi)^{0}$ amplitudes as well as $t'$\change{}{,} and extract information on
  resonances in both the $(3\pi)^{-1}$ and $(2\pi)^{0}$ system and
  their interrelation\change{.}{;}
\item perform a \change{CPV}{$C\!P$ violation} analysis of D and
  B-decays using purely hadronic decays on the level of physical
  amplitudes, instead of in bins within a Dalitz-plot. Such
  \change{CPV}{a $C\!P$ violation} analysis would also
  \change{include}{be based on} the evolution of amplitudes with decay
  time and thus \change{and thus}{} \change{would only work on real
    and imaginary part of the amplitudes and not on event
    numbers}{requires the correct description of the real and
    imaginary part of the amplitudes, not just their magnitude}\change{.}{;}
\item extend all analyses to true 4-body and possibly 5-body final
  states\change{}{.}
\end{itemize}

\subsubsection{Description of a resonance - poles}
Until recent\change{ly}, almost all determinations of meson resonances
and their parameters as well as for heavy baryons \change{are}{have
  been} performed using ``simple'' mass fits comprising Breit-Wigner
amplitudes together with a coherent background amplitude (the
parametrization of the latter \change{one}{} is mostly empirical).
Mostly elastic scattering has allowed to extract the pole information
in the S-matrix. While experimentalists are exposed to much
\change{critics}{criticism}, \change{little}{few} other methods have
been on the market \change{}{and} easily available. Although BaBar and
COMPASS have started to use polynomials and K-matrix poles for their
fits, this work has not been concluded and there is a
strong\change{}{ly} theorist-dependent formulation of these analytical
functions. \remark{is this `theorist-dependent' deliberate? If so,
  fine. Alternatively, you could write: ``There is significant model
  dependence in the formulation of these analytic functions''} Some
more guidance and a list of ``pros'' and "``cons'' of different
recipes, to which one can refer, would be very helpful. We see this as
the only way to obtain process independent information, also referred
to by the PDG.

\subsubsection{Threshold amplitudes}
With the appearance of $XYZ_{c,b}P_c$-states and also\change{
  lately}{, recently,} the $a_1(1420)$, the question of their nature
dominates the \change{physics discussion}{discussion in hadron
  physics}. This is particularly true for resonance structures
appearing close to thresholds of much lighter meson pairs. Here
triangular or loop diagrams can be calculated (probably up to some
overall amplitude factor) resulting in analytical mass functions,
which could be used by experimentalists in their mass-dependent fits,
replacing the above mentioned pole descriptions. This would complete
the information from all analyses involving new states.\remark{I am not entirely sure I understand what's meant with the last sentence.}

\subsubsection{Non-resonant contribution in diffraction}

Diffraction off nucleons always results in a superposition of
production processes, e.g. ``Pomeron'' exchange and ``Deck'' effect,
where the interaction is modeled to proceed via pion nucleon elastic
scattering (\change{exchange of Reggeon}{Reggeon exchange} at the
nucleon-vertex) followed by the exchange of a pion up to the ``upper''
pion-vertex. Deck is thought to be the most prominent non-resonant
contribution in diffraction.  These production processes have
different dependence on the four-momentum exchange $t'$ (to the target
proton) in the reaction and thus may be disentangled \change{}{by}
performing the analysis at various values of $t'$.

It is also of interest to disentangle resonant and non-resonant
production amplitudes, again giving clear access to resonances without
the \change{need}{use} of a \change{simple}{simplistic}
parametrization of \change{of}{} the \change{latter
  ones}{non--resonant contribution}, which is known to distort
information on resonances. Here, a better model for non--resonant
production is required, which could be developed only if detailed
information from ``inside'' the production amplitude is known. This
task should be addressed jointly by theorists and experimentalists.

\subsection{Conclusion}
\change{PWA analysis}{Partial wave analyses} of various multi-body
\change{physics}{} systems have reached a new level of accuracy and
complexity. This allows much closer links with theoretical
calculations and the extraction of physics information could be raised
to a new level, namely (nearly) ``universal'' amplitudes. Extraction
of pole parameters, the role of underlying dynamics and CP violation
based on calculable strong amplitudes could be much rewarding
results. We are aware that \change{many efforts are}{substantial
  effort is} ongoing already (see e.g. ``white
paper''~\cite{Battaglieri:2014gca},
%\footnote{M. Battaglieri et al.,``Analysis Tools for Next-Generation Hadron Spectroscopy Experiments'', Acta Phys.Polon. B46 (2015) 257,  arXiv:1412.6393 [hep-ph]}) 
but a worldwide coherent program, which includes heavy and light quark
physics processes, could accelerate the development, for which theory
is an absolutely necessary and crucial ingredient.



==> bib.tex <==
\begin{thebibliography}{99}

% B2Dhh refs.

\bibitem{lhcb3} 
  R.~Aaij {\it et al.} [LHCb Collaboration],
  {\em Dalitz plot analysis of $B_s^0 \rightarrow \bar{D}^0 K^- \pi^+$ decays},
  Phys.\ Rev.\ D {\bf 90}, 072003 (2014).
  %[arXiv:1407.7712 [hep-ex]].
  %%CITATION = ARXIV:1407.7712;%%
\vskip .2cm

\bibitem{lhcb4} 
  R.~Aaij {\it et al.} [LHCb Collaboration],
  {\em First observation and amplitude analysis of the $B^{-}\to D^{+}K^{-}\pi^{-}$ decay},
  Phys.\ Rev.\ D {\bf 91}, 092002 (2015).
  %[arXiv:1503.02995 [hep-ex]].
  %%CITATION = ARXIV:1503.02995;%%
\vskip .2cm

\bibitem{lhcb5}
  R.~Aaij {\it et al.} [LHCb Collaboration],
  {\em Dalitz plot analysis of $B^0 \to \overline{D}{}^0 \pi^+\pi^-$ decays},
  Phys.\ Rev.\ D {\bf 92}, 032002 (2015).
  %[arXiv:1505.01710 [hep-ex]].
  %%CITATION = ARXIV:1505.01710;%%

\vskip .2cm
\bibitem{lhcb6} 
  R.~Aaij {\it et al.} [LHCb Collaboration],
 {\em Amplitude analysis of $B^0 \rightarrow \bar{D}^0 K^+ \pi^-$ decays},
  Phys.\ Rev.\ D {\bf 92}, 012012 (2015).
  %[arXiv:1505.01505 [hep-ex]].
  %%CITATION = ARXIV:1505.01505;%%

\vskip .2cm
\bibitem{tim1} 
  T.~Gershon,
 {\em On the Measurement of the Unitarity Triangle Angle $\gamma$ from $B^0 \to DK^{*0}$ Decays},
  Phys.\ Rev.\ D {\bf 79}, 051301 (2009).
  %[arXiv:0810.2706 [hep-ph]].
  %%CITATION = ARXIV:0810.2706;%%
  %30 citations counted in INSPIRE as of 24 août 2015
\vskip .2cm
\bibitem{tim2} 
  T.~Gershon and M.~Williams,
  {\em Prospects for the Measurement of the Unitarity Triangle Angle $\gamma$ from 
$B^0 \to DK^+ \pi-$ Decays},
  Phys.\ Rev.\ D {\bf 80}, 092002 (2009).
  %[arXiv:0909.1495 [hep-ph]].
  %%CITATION = ARXIV:0909.1495;%%

\vskip .2cm
\bibitem{tom} 
  T.~Latham and T.~Gershon,
  {\em A Method to Measure $\cos(2\beta)$ Using Time-Dependent Dalitz Plot Analysis of 
$B^0 \to D(CP) \pi^+ \pi^-$},
  J.\ Phys.\ G {\bf 36}, 025006 (2009).
  %[arXiv:0809.0872 [hep-ph]].
  %%CITATION = ARXIV:0809.0872;%%
  %10 citations counted in INSPIRE as of 24 août 2015

\vskip .2cm
\bibitem{beta} 
  J.~Charles, A.~Le Yaouanc, L.~Oliver, O.~Pene and J.~C.~Raynal,
  {\em $B^0_d(t) \to DPP$ time-dependent Dalitz plots, CP-violating angles $2\beta$, $2\beta + \gamma$, 
and discrete ambiguities},
  Phys.\ Lett.\ B {\bf 425}, 375 (1998).
  %[Phys.\ Lett.\ B {\bf 433}, 441 (1998)]
  %[hep-ph/9801363].
  %%CITATION = HEP-PH/9801363;%%
  %85 citations counted in INSPIRE as of 24 août 2015


% B2hhh refs.
\vskip .2cm
\bibitem{expnew} R. Aaij {\em et al.} [LHCb collaboration], {\em Measurements of CP violation
in the three-body phase space of charmless $B^{\pm}$ decays}, 
 Phys. Rev. {\bf D} 90, 112004 (2014).

\vskip .2cm 
\bibitem{babar} B. Aubert  {\em et al.} [BaBar collaboration], 
{\em Search for CP Violation in Neutral D Meson Cabibbo-suppressed Three-body Decays}, 
 Phys. Rev. D {\bf 78}, 101102(R) (2008);  arXiv:0802.4035.

 \vskip .2cm
\bibitem{miranda1} I. Bediaga,  I. I. Bigi, A. Gomes, G. Guerrer, J. Miranda, and A. C. dos Reis, 
{\em On a CP anisotropy measurement in the Dalitz plots}, Phys. Rev. D {\bf 80}, 096006 (2009); 
arXiv:0905.4233[hep-ph].

\vskip .2cm
\bibitem{miranda2} I. Bediaga, J. Miranda, A. C. dos Reis, I. I. Bigi, A. Gomes, J. M. Otalora Goicochea, and A. Veiga,  
{\em Second Generation of Miranda procedure for CP violation in Dalitz studies of B (and D and $\tau$) decays}, Phys. Rev. D {\bf 86}, 036005 (2012); arXiv:1205.3036.

\vskip .2cm
\bibitem{BedPRD14} I. Bediaga, T. Frederico and O. Louren\c{c}o, {\it $CP$ violation and 
$CPT$ invariance in ${B}^{\ifmmode\pm\else\textpm\fi{}}$ decays with final state 
interactions}, Phys. Rev. D {\bf 89}, 094013 (2014).

\vskip .2cm
\bibitem{NogPRD15} J. H. Alvarenga Nogueira, I. Bediaga, A.B.R. Cavalcante, T. Frederico, O. Louren\c co, 
{\it CP violation: Dalitz interference, CPT and FSI }, Phys. Rev. D  {\bf 92}, 054010 (2015).
 
\vskip .2cm
\bibitem{dkpipi1} P. C. Magalh\~aes, M. R. Robilotta, K. S. F. F. Guimar\~aes, 
T. Frederico, W. de Paula, I. Bediaga, A. C. dos Reis, C. M. Maekawa, and G. R. S. 
Zarnauskas, {\it Towards three-body unitarity in 
${D}^{+}\rightarrow{K}^{-}{\pi{}}^{+}{\pi}^{+}$}, Phys. Rev. D {\bf 84}, 094001 (2011).

\vskip .2cm
\bibitem{dkpipi2} K. S. F. F. Guimar\~aes, O. Louren\c{c}o, W. de Paula, T. Frederico and 
A. C. dos Reis, {\it Final state interaction in 
${D}^{+}\rightarrow{K}^{-}{\pi}^{+}{\pi}^{+}$ with $K\pi$ I = 1/2 and 3/2 channels}, J. 
High Energy Phys. 08, 135 (2014).

\vskip .2cm
\bibitem{dkpipi3} T. Frederico, K. S. F. F. Guimar\~aes, O. Louren\c{c}o, W. de Paula, I. 
Bediaga, and A. C. dos Reis, {\it Heavy Meson Decay in Three-Mesons and FSI}, Few Body 
Syst. {\bf 55}, 441 (2014).


% D2hhh refs
\vskip .2cm
\bibitem{kppe791}  E. M. Aitala {\em et al.}, [E791 collaboration],	
{\em Dalitz plot analysis of the $D^+ \to K^-\pi^+\pi^+$  decay  and indication of 
a low-mass scalar $K\pi$ resonance}, Phys. Rev. Lett. {\bf 89}, 121801 (2002).

\vskip .2cm
\bibitem{d3pi-e791}  E. M. Aitala {\em et al.}, [E791 collaboration],
{\em Experimental evidence for a light and broad scalar resonance in
$D^+ \to \pi^-\pi^+\pi^+$  decay}, Phys. Rev. Lett. {\bf 86}, 770 (2001).

\vskip .2cm
\bibitem{ds3pi-e791}  E. M. Aitala {\em et al.}, [E791 collaboration],
{\em Study of the $D^+_s \to \pi^-\pi^+\pi^+$  decay and measurement of the
$f_0$ masses and widths}, Phys. Rev. Lett. {\bf 86}, 765 (2001).

\vskip .2cm
\bibitem{focus-3pi} J. M. Link {\em et al.}, [FOCUS collaboration],
{\em Dalitz plot analysis of $D_s^+$ and $D^+$ decay to $\pi^-\pi^+\pi^+$ using the 
K-matrix formalism}, Phys. Lett. B {\bf 585}, 200 (2004).

\vskip .2cm
\bibitem{d3pi-cleo} G. Bonvicini {\em et al.}, [CLEO collaboration],
{\em Dalitz plot analysis of the $D^+ \to \pi^-\pi^+\pi^+$  decay}, 
Phys. Rev. D {\bf 76}, 012001 (2007).

\vskip .2cm
\bibitem{asner} D. Asner, {\em Charm Dalitz plot analysis formalism and results}, 
arXiv:hep-ex/0410014v3 (2004).

\vskip .2cm
\bibitem{sarantsev} V. V. Anisovich and A. V. Sarantsev, {\em K-matrix analysis of the 
($IJ^{PC}=0^{++}$) wave in the mass region below 1900 MeV},
Eur. Phys. J. {\bf A}16 229, (2003);
arXiv:hep-ph/0204328.

\vskip .2cm
\bibitem{brian} E. M. Aitala {\em et al.},  [E791 collaboration],
{\em Model-independent measurement of the S-wave $K^-\pi^+$ systems using 
$D^+ \to K^-\pi^+\pi^+$ decays from Fermilab E791}, 
Phys. Rev. D {\bf 73}, 032004 (2006).

\vskip .2cm
\bibitem{antimo} B. Aubert {\em et al.},  [BaBar collaboration],
{\em Dalitz plot analysis of the  $D^+_s \to \pi^-\pi^+\pi^+$  decay},
Phys. Rev. D {\bf 79}, 032003 (2009).

\vskip .2cm
\bibitem{cern-munich} B. Hyams {\em et al.}, 
{\em $\pi\pi$ phase-shift analysis from 600 to 1900 MeV}, 
Nucl. Phys. {\bf B64}, 134 (1973);
G. Grayer  {\em et al.}, 
{\em High statistics study of the reaction $\pi^-p\to\pi^-\pi^+n$: Apparatus, method of analysis, 
and general features of results at 17 GeV/c},
Nucl. Phys. {\bf B75}, 189 (1974).

\vskip .2cm
\bibitem{lass} D. Aston {\em et al.},  [LASS collaboration], 
{\em  A study of $K^-\pi^+$ scattering in he reaction $K^-\pi^+\to K^-\pi^+ n$ at 11 GeV},
Nucl. Phys. {\bf B296}, 493 (1988).

\vskip .2cm
\bibitem{watson} K. M. Watson, {\em The effect of final state interactions on 
reaction cross sections}, Phys. Rev.{\bf 88}, 1163 (1952).

\vskip .2cm
\bibitem{focuspwa} J. M . Link  {\em et al.} , [FOCUS collaboration], 
{\em The  $K^-\pi^+$ S-wave from the $D^+ \to K^-\pi^+\pi^+$ decay}, 
 Phys. Lett. {\bf B}681, 14 (2009).

\vskip .2cm
\bibitem{pat} P. C. Magalhães and M. R. Robilotta, 
{\em  $D^+ \to K^-\pi^+\pi^+$: the weak vector current},
Phys. Rev. D {\bf 92}, 094005 (2015); arXiv:1504.06346.

\vskip .2cm
\bibitem{achasov} N.N. Achasov, S.A. Devyanin and G.N. Shestakov,
{\em $S^*-\delta^0$ mixing as a threshold phenomenon},
 Phys. Lett. {\bf B}88, 368 (1979).


% Tomasz refs
\vskip .2cm
\bibitem{LHCb-PAPER-2014-012} R.~Aaij {\it et al.} [LHCb Collaboration],
{\em Measurement of the resonant and CP components in $\overline{B}^0 \to J/\psi\pi^+\pi^-$ decays},Phys. Rev. D{\bf 90},  012003 (2014);
arXiv:1404.5673.

\vskip .2cm
\bibitem{LHCb-PAPER-2013-001} R.~Aaij {\it et al.} [LHCb collaboration],
{\em Determination of the X(3872) meson quantum numbers},
Phys. Rev. Lett. {\bf 110}, 222001 (2013);
arXiv:1302.6269.

\vskip .2cm
\bibitem{LHCb-PAPER-2015-015} R.~Aaij {\it et al.} [LHCb collaboration],
{\em Quantum numbers of the X(3872) state and orbital angular momentum in its $\rho^0 J/\psi$ decays},
arXiv:1504.06339

\vskip .2cm
\bibitem{Bugg:2008wu} D. V. Bugg, 
{\em How Resonances can synchronise with Thresholds},
J. Phys. {\bf G35}, 075005 (2008);
arXiv:0802.0934.

\vskip .2cm
\bibitem{Esposito:2014rxa} A. Esposito {\it et al}, 
{\em Four-Quark Hadrons: an Updated Review},
Int. J. Mod. Phys. {\bf A30}, 1530002 (2014); 
arXiv:1411.5997.

\vskip .2cm
\bibitem{LHCb-PAPER-2014-014} R.~Aaij {\it et al.} [LHCb collaboration],
{\em Observation of the resonant character of the Z(4430)$^-$ state}
Phys. Rev. Lett. {\bf 112}, 222002 (2014); 
arXiv:1404.1903.

\vskip .2cm
\bibitem{Choi:2007wga} S. K. Choi {\it et al.} [Belle collaboration],
{\em Observation of a resonance-like structure in the $\pi^{\pm}\psi'$ mass distribution in 
exclusive $B\to K\pi^{\pm}\psi'$ decays}
Phys. Rev. Lett. {\bf 100}, 142001 (2008); 
arXiv:0708.1790.

\vskip .2cm
\bibitem{Aubert:2008aa}  B. Aubert {\it et al.} [BaBar collaboration],
{\em Search for the Z(4430)$^-$ at BaBar},
Phys. Rev. D {\bf 79}, 112001 (2009); 
arXiv:0811.0564.

\vskip .2cm
\bibitem{Chilikin:2013tch} K. Chilikin {\em et al.} [Belle collaboration],
{\em Experimental constraints on the spin and parity of the Z(4430)$^+$}
Phys. Rev. D {\bf 88}, 074026 (2013); 
arXiv:1306.4894.

\vskip .2cm
\bibitem{Pakhlov:2014qva} P. Pakhlov and T. Uglov,
{\em Charged charmonium-like Z(4430)$^+$ from rescattering in
conventional B decays},
Phys. Lett. B {\bf 748}, 183 (2015); 
arXiv:1408.5295.

\vskip .2cm
\bibitem{LHCb-PAPER-2015-029} R.~Aaij {\it et al.} [LHCb collaboration],
{\em Observation of $J/\psi p$ resonances consistent with pentaquark states in $\Lambda_b^0 \to
J/\psi K^- p$ decays}
Phys. Rev. Lett. {\bf 115}, 072001 (2015);
arXiv:1507.03414.

\vskip .2cm
\bibitem{Maiani:2015vwa} L. Maiani, A. D. Polosa, and V. Riquer,
{\em The New Pentaquarks in the Diquark Model}, 
Phys. Lett. B {\bf 749}, 289 (2015); 
arXiv:1507.04980.

\vskip .2cm
\bibitem{Lebed:2015tna} R. F. Lebed, 
{\em The Pentaquark Candidates in the Dynamical Diquark Picture},
Phys. Lett. B {\bf 749}, 454 (2015);
arXiv:1507.05867.

\vskip .2cm
\bibitem{Anisovich:2015cia} V. V. Anisovich {\em et al.},
{\em Pentaquarks and resonances in the $pJ/\psi$ spectrum};
arXiv:1507.07652.

\vskip .2cm
\bibitem{Karliner:2015ina} M. Karliner and J. L. Rosner,
{\em New Exotic meson and baryon resonances from doubly-heavy hadronic molecules},
Phys. Rev. Lett. {\bf 115} 122001, (2015);
arXiv:1506.06386.

\vskip .2cm
\bibitem{Chen:2015loa} R. Chen, X. Liu, X.-Q. Li, and S.-L. Zhu,
{\em Identifying exotic hidden-charm pentaquarks}
Phys. Rev. Lett. {\bf 115} 132002, (2015);
arXiv:1507.04249.

\vskip .2cm
\bibitem{Roca:2015dva} L. Roca, J. Nieves, and E. Oset,
{\em The LHCb pentaquark as a $\overline{D}^*\Sigma_c-\overline{D}^*\Sigma_c^*$ molecular state}, 
arXiv:1507.04249.

\vskip .2cm
\bibitem{He:2015cea} J. He,
{\em $\overline{D}^*\Sigma_c$ and  $\overline{D}\Sigma_c^*$ interactions and the LHCb 
hidden-charmed pentaquarks},
arXiv:1507.05200.

\vskip .2cm
\bibitem{Meissner:2015mza} U.-G. Meissner and J. A. Oller,
{\em Testing the $\chi_{c1} p$ composite nature of the $P_c(4450)$},
arXiv:1507.07478.

\vskip .2cm
\bibitem{Liu:2015fea} X.-H. Liu, Q. Wang, and Q. Zhao,
{\em Understanding the newly observed heavy pentaquark candidates}, 
arXiv:1507.05359.

\vskip .2cm
\bibitem{Mikhasenko:2015vca} M. Mikhasenko,
{\em A triangle singularity and the LHCb pentaquarks}, 
arXiv:1507.06552.
\vskip .2cm
\bibitem{Szczepaniak:2015hya} A. P. Szczepaniak,
{\em Dalitz plot distributions in presence of triangle singularities,}
arXiv:1510.01789.

\vskip .2cm
\bibitem{Aaij:2015zxa} R.~Aaij {\it et al.} [LHCb Collaboration],
{\em A model-independent confirmation of the Z(4430)$^-$}, 
arXiv:1510.01951.

% Diogo's references
\vskip .2cm
\bibitem{Beneke2003} M.~Beneke and M.~Neubert,
\textit{QCD factorization for $B\to PP$ and $B\to PV$ decays}, 
Nucl. Phys. B \textbf{675}, 333 (2003).

\vskip .2cm
\bibitem{Bauer1987} 
M. Bauer, B. Stech and M. Wirbel,
\textit{Exclusive Non-Leptonic Decays of $D$, $D_s$ and $B$-Mesons},
Z. Phys. C {\bf 34}, 103 (1987).

\vskip .2cm
\bibitem{Abbasetal} 
  A.~Biswas, N.~Sinha and G.~Abbas,
 \textit{Nonleptonic decays of charmed mesons into two pseudoscalars},
 Phys.\ Rev.\ D {\bf 92},  014032 (2015).

\vskip .2cm
\bibitem{Boitoetal09}D.~R.~Boito, J.-P.~Dedonder, B.~El-Bennich, O.~Leitner and B.~Loiseau,
\textit{Scalar resonances in a unitary $\pi \pi$ S-wave model for $D^+ \to \pi^+ \pi^- \pi^+$},
 Phys.\ Rev.\ D {\bf 79}, 034020 (2009).

\vskip .2cm
\bibitem{BE2009}D.~R.~Boito and R.~Escribano,
\textit{$K\pi$ form-factors and final state interactions in $D^+ \to K^- \pi^+ \pi^+$ decays},
Phys. Rev. D {\bf 80}, 054007 (2009).

\vskip .2cm
\bibitem{ElBennichetal09}B.~El-Bennich, A.~Furman, R.~Kaminski, L.~Lesniak, B.~Loiseau and B.~Moussallam,
\textit{CP violation and kaon-pion interactions in $B \to K \pi^+ \pi^-$ decays},
 Phys.\ Rev.\ D {\bf 79}, 094005 (2009); Erratum-ibid, Phys.\ Rev.\ D {\bf 83}, 039903 (2011)].  

\vskip .2cm
\bibitem{JPD_PRD89}
J.-P. Dedonder, R. R Kami\'nski, L. Le\'sniak and B. Loiseau, 
\textit{Dalitz plot studies of $D^0 \to K_S^0 \pi^+ \pi^-$ decays in a factorization approach},
Phys. Rev. D {\bf 89}, 094018 (2014).

\vskip .2cm
\bibitem{BurasNPB434_606} A. J. Buras, 
\textit{QCD factors $a_1$ and $a_2$ beyond leading logarithms versus factorization in non leptonic heavy meson decays}, Nucl. Phys. B {\bf 434}, 606 (1995).


\bibitem{MG02}  S.~Gardner and U.~G.~Meissner,
\textit{Rescattering and chiral dynamics in $B \to \rho \pi$ decay},
Phys.\ Rev.\ D {\bf 65}, 094004 (2002).

\vskip .2cm
\bibitem{FFs1}  M.~Jamin, J.~A.~Oller and A.~Pich,
\textit{Scalar $K\pi$ form factor and light-quark masses}, Phys.\ Rev.\ D {\bf 74}, 074009  (2006).

\vskip .2cm
\bibitem{FFs2} B.~Moussallam, 
\textit{Analyticity constraints on the strangeness changing vector current and applications 
to $\tau \to K\pi\nu_{\tau}$ and $\tau\to K\pi\pi\nu_{\tau}$},
Eur.\ Phys.\ J.\ C {\bf 53}, 401 (2008).

\vskip .2cm
\bibitem{FFs3}D.~R.~Boito, R.~Escribano and M.~Jamin,
\textit{$K\pi$ vector form factors constrained by $\tau \to K \pi \nu_\tau$ and  $K_{l3}$ decays},
 J. High Energy Phys. {\bf 1009}, 031 (2010).

\vskip .2cm
\bibitem{Melikhov}
D.~Melikhov, 
\textit{Dispersion approach to quark-binding effects in weak decays of heavy mesons},
Eur.\ Phys.\ J.\ direct C {\bf 4}, C2 (2002); arXiv:hep-ph/0110087.


% LONDON's references
\vskip .2cm
\bibitem{BPPP_FS}
B.~Bhattacharya, M.~Gronau, M.~Imbeault, D.~London and J.~L.~Rosner,
  {\em Charmless $B\to PPP$ decays: The fully-symmetric final state},
  Phys.\ Rev.\ D {\bf 89}, no. 7, 074043 (2014);
  arXiv:1402.2909.
  %%CITATION = ARXIV:1402.2909;%%


\bibitem{MGUspin} 
M.~Gronau,
  {\em U spin symmetry in charmless B decays},
  Phys.\ Lett.\ B {\bf 492}, 297 (2000);
  hep-ph/0008292.
  %%CITATION = HEP-PH/0008292;%%


\bibitem{BPPPgamma1}
N.~Rey-Le Lorier and D.~London,
  {\em Measuring gamma with $B \to K \pi \pi$ and $B \to K K \bar{k}$ Decays},
  Phys.\ Rev.\ D {\bf 85}, 016010 (2012);
  arXiv:1109.0881.
  %%CITATION = ARXIV:1109.0881;%%


\bibitem{BPPPgamma2}
B.~Bhattacharya, M.~Imbeault and D.~London,
  {\em Extraction of the CP-violating phase $\gamma$ using $B \to K \pi \pi$ and $B \to K K \bar K$ decays},
  Phys.\ Lett.\ B {\bf 728}, 206 (2014); arXiv:1303.0846.
  %%CITATION = ARXIV:1303.0846;%%


\bibitem{BPPPdiagrams} 
N.~Rey-Le Lorier, M.~Imbeault and D.~London,
  {\em Diagrammatic Analysis of Charmless Three-Body B Decays},
  Phys.\ Rev.\ D {\bf 84}, 034040 (2011);
  arXiv:1011.4972.
  %%CITATION = ARXIV:1011.4972;%%


\vskip .2cm
% OSET's references
%\cite{Oller:1997ti}
\bibitem{npa}
  J.~A.~Oller and E.~Oset,
  {\em Chiral symmetry amplitudes in the S wave isoscalar and isovector channels and the $\sigma$, 
$f_0(980)$, $a_0(980)$ scalar mesons},
  Nucl.\ Phys.\ A {\bf 620}, 438 (1997),
  [Erratum-ibid.\ A {\bf 652}, 407 (1999)].
%  [hep-ph/9702314].
  %%CITATION = HEP-PH/9702314;%%
  %471 citations counted in INSPIRE as of 21 Jun 2014

%\cite{Oller:1998hw}
\vskip .2cm
\bibitem{ramonet}
  J.~A.~Oller, E.~Oset and J.~R.~Pelaez,
  {\em Meson meson interaction in a nonperturbative chiral approach},
  Phys.\ Rev.\ D {\bf 59}, 074001 (1999), 
  [Erratum-ibid.\ D {\bf 60}, 099906 (1999)], 
  [Erratum-ibid.\ D {\bf 75}, 099903 (2007)];
  hep-ph/9804209.
  %%CITATION = HEP-PH/9804209;%%
  %455 citations counted in INSPIRE as of 21 Jun 2014

\vskip .2cm
%\cite{Liang:2014tia}
\bibitem{liang} 
  W.~H.~Liang and E.~Oset,
  {\em $B^0$ and $B^0_s$ decays into $J/\psi$ $f_0(980)$ and $J/\psi$ $f_0(500)$ and the nature of the scalar resonances},
  Phys.\ Lett.\ B {\bf 737}, 70 (2014);
  arXiv:1406.7228 [hep-ph].
  %%CITATION = ARXIV:1406.7228;%%
  %16 citations counted in INSPIRE as of 17 Aug 2015

\vskip .2cm
%\cite{Xie:2014tma}
\bibitem{dai} 
  J.~J.~Xie, L.~R.~Dai and E.~Oset,
  {\em The low lying scalar resonances in the $D^0$ decays into $K^0_s$ and $f_0(500)$, $f_0(980)$, $a_0(980)$},
  Phys.\ Lett.\ B {\bf 742}, 363 (2015);
  arXiv:1409.0401 [hep-ph].
  %%CITATION = ARXIV:1409.0401;%%
  %5 citations counted in INSPIRE as of 17 Aug 2015

\vskip .2cm
 %\cite{Weinberg:1978kz}
\bibitem{Weinberg:1978kz} 
  S.~Weinberg,
 {\em Phenomenological Lagrangians},
  Physica A {\bf 96}, 327 (1979).
  %%CITATION = PHYSA,A96,327;%%

 \vskip .2cm
%\cite{Gasser:1983yg}
\bibitem{Gasser:1983yg} 
  J.~Gasser and H.~Leutwyler,
  {\em Chiral Perturbation Theory to One Loop},
  Annals Phys.\  {\bf 158}, 142 (1984).
  %%CITATION = APNYA,158,142;%%

\vskip .2cm
%\cite{Bando:1987br}
\bibitem{bando} 
  M.~Bando, T.~Kugo and K.~Yamawaki,
  {\em Nonlinear Realization and Hidden Local Symmetries},
  Phys.\ Rept.\  {\bf 164}, 217 (1988).
  %%CITATION = PRPLC,164,217;%%
  %937 citations counted in INSPIRE as of 20 août 2015

\vskip .2cm
%\cite{vanBeveren:1986ea}
\bibitem{vanBeveren:1986ea} 
  E.~van Beveren, T.~A.~Rijken, K.~Metzger, C.~Dullemond, G.~Rupp and J.~E.~Ribeiro,
  {\em A Low Lying Scalar Meson Nonet in a Unitarized Meson Model},
  Z.\ Phys.\ C {\bf 30}, 615 (1986).
  %%CITATION = ARXIV:0710.4067;%%
  %385 citations counted in INSPIRE as of 19 Aug 2015

\vskip .2cm
%\cite{Tornqvist:1995ay}
\bibitem{Tornqvist:1995ay} 
  N.~A.~Tornqvist and M.~Roos,
  {\em Resurrection of the sigma meson},
  Phys.\ Rev.\ Lett.\  {\bf 76}, 1575 (1996);
  hep-ph/9511210.
  %%CITATION = HEP-PH/9511210;%%
  %390 citations counted in INSPIRE as of 19 Aug 2015

\vskip .2cm
%\cite{Fariborz:2009cq}
\bibitem{Fariborz:2009cq} 
  A.~H.~Fariborz, R.~Jora and J.~Schechter,
  {\em Global aspects of the scalar meson puzzle},
  Phys.\ Rev.\ D {\bf 79}, 074014 (2009);
  arXiv:0902.2825 [hep-ph].
  %%CITATION = ARXIV:0902.2825;%%
  %53 citations counted in INSPIRE as of 19 août 2015

\vskip .2cm
%\cite{Fariborz:2009wf}
\bibitem{Fariborz:2009wf} 
  A.~H.~Fariborz, N.~W.~Park, J.~Schechter and M.~Naeem Shahid,
  {\em `Gauged linear sigma model and pion-pion scattering},
  Phys.\ Rev.\ D {\bf 80}, 113001 (2009); 
  arXiv:0907.0482 [hep-ph].
  %%CITATION = ARXIV:0907.0482;%%
  %11 citations counted in INSPIRE as of 19 Aug 2015

\vskip .2cm
%\cite{Gamermann:2006nm}
\bibitem{gamermann} 
  D.~Gamermann, E.~Oset, D.~Strottman and M.~J.~Vicente Vacas,
  {\em Dynamically generated open and hidden charm meson systems},
  Phys.\ Rev.\ D {\bf 76}, 074016 (2007); 
  hep-ph/0612179.
  %%CITATION = HEP-PH/0612179;%%
  %130 citations counted in INSPIRE as of 17 Aug 2015

\vskip .2cm
%\cite{Gamermann:2007mu}
\bibitem{danires} 
  D.~Gamermann and E.~Oset,
 {\em Hidden charm dynamically generated resonances and the $e^+ e^- \to J/\psi D \bar D, 
/\psi D \bar D^*$ reactions},
  Eur.\ Phys.\ J.\ A {\bf 36}, 189 (2008); 
  arXiv:0712.1758 [hep-ph].
  %%CITATION = ARXIV:0712.1758;%%
  %38 citations counted in INSPIRE as of 17 Aug 2015

\vskip .2cm
%\cite{Albaladejo:2015kea}
\bibitem{miguel} 
  M.~Albaladejo, M.~Nielsen and E.~Oset,
   {\em $D_{s0}^{\ast\pm}(2317)$ and $KD$ scattering from $B^0_s$ decay},
  Phys.\ Lett.\ B {\bf 746}, 305 (2015); 
  arXiv:1501.03455 [hep-ph].
  %%CITATION = ARXIV:1501.03455;%%
  %3 citations counted in INSPIRE as of 17 Aug 2015

\vskip .2cm
%\cite{Navarra:2015iea}
\bibitem{sekihara} 
  F.~S.~Navarra, M.~Nielsen, E.~Oset and T.~Sekihara,
   {\em Testing the molecular nature of $D_{s0}^*(2317)$ and $D_0^*(2400)$ in semileptonic $B_s$ and $B$ decays},
  Phys.\ Rev.\ D {\bf 92}, no. 1, 014031 (2015)
  arXiv:1501.03422 [hep-ph].
  %%CITATION = ARXIV:1501.03422;%%
  %4 citations counted in INSPIRE as of 17 Aug 2015

\vskip .2cm
%\cite{Liang:2015twa}
\bibitem{liangxyz} 
  W.~H.~Liang, J.~J.~Xie, E.~Oset, R.~Molina and M.~Döring,
   {\em Predictions for the $\bar B^0 \to \bar K^{*0} X (YZ)$ and $\bar B^0_s \to \phi X (YZ)$ with $X(4160), Y(3940), Z(3930)$},
  Eur.\ Phys.\ J.\ A {\bf 51}, no. 5, 58 (2015); 
  arXiv:1502.02932 [hep-ph].
  %%CITATION = ARXIV:1502.02932;%%

\vskip .2cm
%\cite{Aaij:2015tga}
\bibitem{penta} 
  R.~Aaij {\it et al.} [LHCb Collaboration],
   {\em Observation of $J/\psi p$ resonances consistent with pentaquark states in ${\Lambda_b^0\to J/\psi K^-p}$ decays},
  Phys.\ Rev.\ Lett.\  {\bf 115}, 072001 (2015); 
  arXiv:1507.03414 [hep-ex].
  %%CITATION = ARXIV:1507.03414;%%
  %24 citations counted in INSPIRE as of 17 Aug 2015



%RUPP's references
\vskip .2cm
\bibitem{PLB63p224}
S.~M.~Flatte,
 {\em Coupled - Channel Analysis of the $\pi \eta$ and $K\bar K$ Systems Near $K\bar K$
 Threshold},
Phys.\ Lett.\ B {\bf 63}, 224 (1976).
%%CITATION = PHLTA,B63,224;%%

\vskip .2cm
\bibitem{Appel01}
Jeffrey A.\ Appel, private communications (2001).

\vskip .2cm
\bibitem{EPJC10p469}
E.~van Beveren and G.~Rupp,
 {\em Comment on `Understanding the scalar meson $q\bar q$ nonet'},
Eur.\ Phys.\ J.\ C {\bf 10}, 469 (1999); 
arXiv:hep-ph/9806246.
%%CITATION = HEP-PH/9806246;%%

\vskip .2cm
\bibitem{ZPC68p647}
N.~A.~Tornqvist,
{\em Understanding the scalar meson $q\bar q$ nonet},
Z.\ Phys.\ C {\bf 68}, 647 (1995); 
arXiv:hep-ph/9504372.
%%CITATION = HEP-PH/9504372;%%

\vskip .2cm
\bibitem{PRL76p1575}
N.~A.~Tornqvist and M.~Roos,
{\em Resurrection of the sigma meson},
Phys.\ Rev.\ Lett.\ {\bf 76}, 1575 (1996); 
arXiv:hep-ph/9511210.
%%CITATION = HEP-PH/9511210;%%

\vskip .2cm
\bibitem{ZPC30p615}
E.~van Beveren, T.~A.~Rijken, K.~Metzger, C.~Dullemond, G.~Rupp,
and J.~E.~Ribeiro,
{\em A Low Lying Scalar Meson Nonet in a Unitarized Meson Model},
Z.\ Phys.\ C {\bf 30}, 615  (1986);
arXiv:0710.4067 [hep-ph].
%%CITATION = ARXIV:0710.4067;%%

\vskip .2cm
\bibitem{EPJC22p493}
E.~van Beveren and G.~Rupp,
{\em Modified Breit-Wigner formula for mesonic resonances describing OZI decays
of confined $q\bar q$ states and the light scalar mesons},
Eur.\ Phys.\ J.\ C {\bf 22}, 493 (2001); 
arXiv:hep-ex/0106077.
%%CITATION = HEP-EX/0106077;%%

\vskip .2cm
\bibitem{IJTPGTNLO11p179}
E.~van Beveren and G.~Rupp,
{\em Reconciling the light scalar mesons with Breit-Wigner resonances as well as
 the quark model},
Int.\ J.\ Theor.\ Phys.\ Group Theor.\ Nonlin.\ Opt.\  {\bf 11}, 179  (2006);
arXiv:hep-ph/0304105.
%%CITATION = HEP-PH/0304105;%%

\vskip .2cm
\bibitem{PRL91p012003}
E.~van Beveren and G.~Rupp,
{\em Observed $D_s(2317)$ and tentative D(2030) as the charmed cousins of the
 light scalar nonet},
Phys.\ Rev.\ Lett.\  {\bf 91}, 012003 (2003); 
arXiv:hep-ph/0305035]
%%CITATION = HEP-PH/0305035;%%

\vskip .2cm
\bibitem{PLB641p265}
E.~van Beveren, D.~V.~Bugg, F.~Kleefeld,\ and G.~Rupp,
 {\em The Nature of $\sigma$, $\kappa$, $a_0(980)$ and $f_0(980)$},
Phys.\ Lett.\ B {\bf 641}, 265 (2006); 
arXiv:hep-ph/0606022.
%%CITATION = HEP-PH/0606022;%%

\vskip .2cm
\bibitem{PRL97p202001}
E.~van Beveren and G.~Rupp,
 {\em New BABAR state D(sJ) (2860) as the first radial excitation of the
 $D^*_{(s0)} (2317)$},
Phys.\ Rev.\ Lett.\ {\bf 97}, 202001 (2006); 
arXiv:hep-ph/0606110.
%%CITATION = HEP-PH/0606110;%%
 {\em Comment on `Study of $D_{(sJ)}$ decays to $D^*K$ in inclusive
$e^+ e^-$ interactions'},
Phys.\ Rev.\ D {\bf 81}, 118101 (2010); 
arXiv:0908.1142 [hep-ph].
%%CITATION = ARXIV:0908.1142;%%

\vskip .2cm
\bibitem{AP324p1620}
E.~van Beveren and G.~Rupp,
{\em Meson-meson interactions and Regge propagators},
Annals Phys.\ {\bf 324}, 1620  (2009);  
arXiv:0809.1149 [hep-ph].
%%CITATION = ARXIV:0809.1149;%%

\vskip .2cm
\bibitem{PRD84p094020}
S.~Coito, G.~Rupp, and E.~van Beveren,
{\em Quasi-bound states in the continuum: a dynamical coupled-channel
 calculation of axial-vector charmed mesons},
Phys.\ Rev.\ D {\bf 84}, 094020 (2011); 
arXiv:1106.2760 [hep-ph].
%%CITATION = ARXIV:1106.2760;%%

\vskip .2cm
\bibitem{EPJC71p1762}
S.~Coito, G.~Rupp, and E.~van Beveren,
{\em Delicate interplay between the $D^0-D^{*0}$, $\rho^0-J/\psi$, and $\omega-J/\psi$ channels
 in the $X(3872)$ resonance},
Eur.\ Phys.\ J.\ C {\bf 71}, 1762; (2011) 
arXiv:1008.5100 [hep-ph].
%%CITATION = ARXIV:1008.5100;%%

\vskip .2cm
\bibitem{ZPC21p291}
E.~van Beveren,
{\em Coupling Constants and Transition Potentials for Hadronic Decay Modes of a Meson},
Z.\ Phys.\ C {\bf 21}, 291 (1984); 
arXiv:hep-ph/0602246.
%%CITATION = HEP-PH/0602246;%%

\vskip .2cm
\bibitem{PRD71p114513}
G.~S.~Bali {\it et al.} [SESAM Collaboration],
{\em Observation of string breaking in QCD},
Phys.\ Rev.\ D {\bf 71}, 114513 (2005); 
arXiv:hep-lat/0505012.
%%CITATION = HEP-LAT/0505012;%%

\vskip .2cm
\bibitem{PDG2014}
K.~A.~Olive {\it et al.} [Particle Data Group Collaboration],
{\em Review of Particle Physics}, 
Chin.\ Phys.\ C {\bf 38}, 090001 (2014).
%%CITATION = CHPHD,C38,090001;%%

\vskip .2cm
\bibitem{AP323p1215}
E.~van Beveren and G.~Rupp,
{\em Relating multichannel scattering and production amplitudes
in a microscopic OZI-based model},
Annals Phys.\ {\bf323}, 1215 (2008);
arXiv:0706.4119 [hep-ph].
%%CITATION = ARXIV:0706.4119;%%

\vskip .2cm
\bibitem{EPL81p61002}
E.~van Beveren and G.~Rupp,
{\em The complex relation between production and scattering amplitudes},
Europhys.\ Lett.\ {\bf 81}, 61002 (2008);
arXiv:0710.5823 [hep-ph].
%%CITATION = EULEE,81,61002;%%

\vskip .2cm
\bibitem{EPL84p51002}
E.~van Beveren and G.~Rupp,
{\em Reply to the comment by M.R. Pennington and D.J. Wilson},
Europhys.\ Lett.\  {\bf 84}, 51002 (2008).
%%CITATION = EULEE,84,51002;%%

\vskip .2cm
\bibitem{EPL84p51001}
M.~R.~Pennington and D.~J.~Wilson,
{\em How adding zero to the complex relation between production and scattering
 amplitudes found by van Beveren and Rupp gives the expected real relation},
Europhys.\ Lett.\ {\bf 84}, 51001 (2008); 
arXiv:0711.3521 [hep-ph].
%%CITATION = ARXIV:0711.3521;%%

\vskip .2cm
\bibitem{EPL85p61002}
E.~van Beveren, X.~Liu, R.~Coimbra and G.~Rupp,
{\em Possible $\psi(5S)$, $\psi(4D)$, $\psi(6S)$ and $\psi(5D)$ signals in 
$\Lambda_c \overline{\Lambda_c}$}, 
Europhys.\ Lett.\ {\bf 85}, 61002 (2009); 
arXiv:0809.1151 [hep-ph].
%%CITATION = ARXIV:0809.1151;%%

\vskip .2cm
\bibitem{PRD80p074001}
E.~van Beveren and G.~Rupp,
{\em Production of hadron pairs in $e^+ e^-$ annihilation near the $K^+K^-$, $D \bar D$,
$B \bar B$ and $\Lambda_c^+\Lambda_c^-$ thresholds},
Phys.\ Rev.\ D {\bf 80}, 074001 (2009); 
arXiv:0908.0242 [hep-ph].
%%CITATION = ARXIV:0908.0242;%%

%Tobias'references
 \vskip .2cm
\bibitem{Marshak} R. E. Marshak, Riazuddin, and C. P. Ryan, {\it Theory of Weak 
Interactions in Particle Physics}, Wiley-Interscience (1969).

\vskip .2cm
\bibitem{Branco} G. C. Branco, L. Lavoura, J. P. Silva, {\it CP Violation}, Oxford 
University Press (1999).

\vskip .2cm
\bibitem{bigibook} I. I. Bigi, A. I. Sanda, {\em  CP Violation}, 2nd Edition, Cambridge 
University Press (2009).

\vskip .2cm
\bibitem{BSS} M. Bander, D. Silverman, A. Soni, {\it $\mathrm{CP}$ Noninvariance in the 
Decays of Heavy Charged Quark Systems}, Phys. Rev. Lett. {\bf 43}, 242 (1979).

\vskip .2cm
\bibitem{Soni2005} D. Atwood, A. Soni, {\it Possibility of large direct $\mathrm{CP}$ 
violation in $\stackrel{\rightarrow}{B}K\pi$-like modes because of long distance 
rescattering effects and implications for the angle $\gamma$}, Phys. Rev.  D {\bf 58},
 036005 (1998); H.-Y. Cheng, C.-K. Chua, A. Soni, {\it Final state interactions in 
hadronic $B$ decays}, Phys. Rev.  D {\bf 71}, 014030 (2005).

\vskip .2cm
\bibitem{wolfenstein} L. Wolfenstein, {\it Final-state interactions and $\mathrm{CP}$ 
violation in weak decays}, Phys. Rev. D {\bf 43}, 151 (1991).

\vskip .2cm
\bibitem{LHCbPRL13} R. Aaij {\it et al.} (LHCb Collaboration), 
{\em Measurement of CP Violation in the Phase Space of $B^{\pm}\to K^{\pm}\pi^+\pi^-$ and 
$B^{\pm}\to K^{\pm}K^+K^-$}
Phys. Rev. Lett. {\bf 111}, 101801 (2013).

\vskip .2cm
\bibitem{Cohen1980} D. Cohen et al., {\it Amplitude analysis of the $K^-K^+$ system 
produced in the reactions $\pi^-$p$\to K^-K^+$n and $K^-K^+$ at 6 GeV/c}, Phys. Rev. D 
{\bf 22}, 2595 (1980).

\vskip .2cm
\bibitem{pelaprd05} J. R. Pel\'aez, F. J. Yndur\'ain, {\it Pion-pion scattering amplitude}, 
Phys. Rev. D {\bf 71}, 074016 (2005);
R. Garc\'ia-Mart\'in, R. Kami\'nski, J.R. Pel\'aez, J. Ruiz de Elvira,  F. J. Yndur\'ain, 
{\em Pion-pion scattering amplitude. IV. Improved analysis with once subtracted Roy-like equations up to 1100 MeV}, 
Phys. Rev. D {\bf 83}, 074004 (2011).

\vskip .2cm
\bibitem{ref8} N. Brambilla {\it et al.} {\it QCD and strongly coupled gauge theories: 
challenges and perspectives}, Eur. Phys. J. C {\bf 74}, 2981 (2014).


%ADAM's references
\vskip .2cm
\bibitem{MartinSpearman} 
A.D. Martin and T.D. Spearman, {\it Elementary Particle Theory}, North-Holland, Amsterdam, and Elsevier, New York, (1970).

\vskip .2cm
\bibitem{Danilkin:2014cra} 
  I.~V.~Danilkin, C.~Fernandez-Ramirez, P.~Guo, V.~Mathieu, D.~Schott, M.~Shi and A.~P.~Szczepaniak,
 {\em Dispersive analysis of $\omega/\phi \to 3\pi,\ \pi \gamma*$},
  Phys.\ Rev.\ D {\bf 91},  094029 (2015);
  arXiv:1409.7708 [hep-ph].
  
\vskip .2cm
 \bibitem{Pham:1976yi} 
  T.~N.~Pham and T.~N.~Truong,
  {\em Muskhelishvili-Omnes Integral Equation with Inelastic Unitarity: Single and Coupled Channel Equations},
  Phys.\ Rev.\ D {\bf 16}, 896 (1977).
  %%CITATION = PHRVA,D16,896;%%
 
\vskip .2cm
 \bibitem{gribov} 
V.N.~Gribov, J.~Nyiri, Y.~Dokshitzer, {\it  Strong interactions of hadrons at high energies : Gribov lectures on theoretical physics}, Cambridge University Press Cambridge, UK, New York (2009). 

\vskip .2cm
\bibitem{Szczepaniak:2015eza} 
  A.~P.~Szczepaniak,
  {\em Triangle Singularities and XYZ Quarkonium Peaks},
  Phys.\ Lett.\ B {\bf 747}, 410 (2015);
  arXiv:1501.01691 [hep-ph].
 
 \vskip .2cm
 \bibitem{schmid}  C. Schmid, {\em Final-State Interactions and the Simulation of Resonances},
 Phys. Rev. 154, 1363 (1964). 
 

%%  Pelaez references
\vskip .2cm
\bibitem{Pelaez:2015qba} 
  J.~R.~Pelaez,
  {\em From controversy to precision on the sigma meson: a review on the status of the non-ordinary $f_0(500)$ resonance},
  arXiv:1510.00653 [hep-ph].
  %%CITATION = ARXIV:1510.00653;%%
  %4 citations counted in INSPIRE as of 20 Oct 2015

\vskip .2cm
%\cite{Pelaez:2013jp}
\bibitem{Pelaez:2013jp} 
  J.~R.~Pelaez,
  {\em Recent progress on light scalars: from confusion to precision using dispersion theory},
  PoS ConfinementX {\bf }, 019 (2012);
  arXiv:1301.4431 [hep-ph].
  %%CITATION = ARXIV:1301.4431;%%
  %16 citations counted in INSPIRE as of 20 Oct 2015

\vskip .2cm
%\cite{Aaij:2013zpt}
\bibitem{Aaij:2013zpt}  
  R.~Aaij {\it et al.} [LHCb Collaboration],
  {\em Analysis of the resonant components in $\overline{B}^0\to J/\psi \pi^+\pi^-$},
  Phys.\ Rev.\ D {\bf 87}, no. 5, 052001 (2013);
  arXiv:1301.5347 [hep-ex].
  %%CITATION = ARXIV:1301.5347;%%
  %37 citations counted in INSPIRE as of 20 Oct 2015

\vskip .2cm
%\cite{Aaij:2014siy}
\bibitem{Aaij:2014siy}
  R.~Aaij {\it et al.} [LHCb Collaboration],
  {\em Measurement of the resonant and CP components in $\overline{B}^0\to J/\psi \pi^+\pi^-$ decays},
  Phys.\ Rev.\ D {\bf 90},  012003 (2014);
  arXiv:1404.5673 [hep-ex].
  %%CITATION = ARXIV:1404.5673;%%
  %36 citations counted in INSPIRE as of 20 Oct 2015


\vskip .2cm
%\cite{Stone}
\bibitem{Stone} 
  S.~Stone and L.~Zhang,
  {\em Use of $B\to J/\psi f_0$ decays to discern the $q \bar{q}$ or tetraquark nature of scalar mesons},
  Phys.\ Rev.\ Lett.\  {\bf 111}, 062001 (2013);
  arXiv:1305.6554 [hep-ex].
  %%CITATION = ARXIV:1305.6554;%%
  %28 citations counted in INSPIRE as of 20 Oct 2015

\vskip .2cm
%\cite{Fleischer:2011au}
\bibitem{Fleischer:2011au} 
  R.~Fleischer, R.~Knegjens and G.~Ricciardi,
  {\em Anatomy of $B^0_{s,d} \to J/\psi f_0(980)$},
  Eur.\ Phys.\ J.\ C {\bf 71}, 1832 (2011);
  arXiv:1109.1112 [hep-ph].
  %%CITATION = ARXIV:1109.1112;%%
  %49 citations counted in INSPIRE as of 20 Oct 2015

\vskip .2cm
\bibitem{PDG} K.A. Olive et al. (Particle Data Group), 
Chin. Phys. C, 38, 090001 (2014) and 2015 update.

\vskip .2cm
%\cite{Cohen:2014vta}
\bibitem{Cohen:2014vta} 
  T.~Cohen, F.~J.~Llanes-Estrada, J.~R.~Pelaez and J.~Ruiz de Elvira,
  {\em Nonordinary light meson couplings and the $1/N_c$ expansion}, 
  Phys.\ Rev.\ D {\bf 90}, no. 3, 036003 (2014);
  arXiv:1405.4831 [hep-ph].
  %%CITATION = ARXIV:1405.4831;%%
  %5 citations counted in INSPIRE as of 20 Oct 2015

\vskip .2cm
%\cite{Liang:2014tia}
\bibitem{Liang:2014tia} 
  W.~H.~Liang and E.~Oset,
  {\em $B^0$ and $B^0_s$ decays into $J/\psi f_0(980)$ and $J/\psi f_0(500)$ and the nature of the scalar resonances},
  Phys.\ Lett.\ B {\bf 737}, 70 (2014);
  arXiv:1406.7228 [hep-ph].
  %%CITATION = ARXIV:1406.7228;%%
  %22 citations counted in INSPIRE as of 20 Oct 2015

\vskip .2cm
\bibitem{weinbergdeuterium}
S. Weinberg, Phys. Rev. {\bf130}, 776 (1963); {\bf 131}, 440 (1963); {\bf 137} B672 (1965).

\vskip .2cm
%\cite{Daub:2015xja}
\bibitem{Daub:2015xja} 
  J.~T.~Daub, C.~Hanhart and B.~Kubis,
  {\em A model-independent analysis of final-state interactions in $\bar B_{d/s}^0 \to J/\psi\pi\pi$},
  arXiv:1508.06841 [hep-ph].
  %%CITATION = ARXIV:1508.06841;%%
  %4 citations counted in INSPIRE as of 20 Oct 2015

\vskip .2cm
%\cite{Brodsky:2014xia}
\bibitem{Brodsky:2014xia} 
  S.~J.~Brodsky, D.~S.~Hwang and R.~F.~Lebed,
  {\em Dynamical Picture for the Formation and Decay of the Exotic XYZ Mesons},
  Phys.\ Rev.\ Lett.\  {\bf 113}, 112001 (2014);
  arXiv:1406.7281 [hep-ph].
  %%CITATION = ARXIV:1406.7281;%%
  %21 citations counted in INSPIRE as of 20 Oct 2015

\vskip .2cm
%\cite{Close}
\bibitem{Close} 
  F.~E.~Close and A.~Kirk,
  {\em Interpretation of scalar and axial mesons in LHCb from a historical perspective},
  Phys.\ Rev.\ D {\bf 91}, no. 11, 114015 (2015);
  arXiv:1503.06942 [hep-ex].
  %%CITATION = ARXIV:1503.06942;%%
  %3 citations counted in INSPIRE as of 20 Oct 2015

\vskip .2cm
%\cite{Close:2002zu}
\bibitem{Close:2002zu} 
  F.~E.~Close and N.~A.~Tornqvist,
  {\em Scalar mesons above and below 1-GeV},
  J.\ Phys.\ G {\bf 28}, R249 (2002);
  hep-ph/0204205.
  %%CITATION = HEP-PH/0204205;%%
  %344 citations counted in INSPIRE as of 20 Oct 2015

\vskip .2cm
%\cite{Howarth:2015caa}
\bibitem{Howarth:2015caa} 
  D.~Howarth and J.~Giedt,
  {\em The sigma meson from lattice QCD with two-pion interpolating operators},
  arXiv:1508.05658 [hep-lat].
  %%CITATION = ARXIV:1508.05658;%%
  %1 citations counted in INSPIRE as of 20 Oct 2015


% Patricia's references
\vskip .2cm
\bibitem{BenoitBppp} J. -P. Dedonder, A. Furman, R.  Kaminski, L. Lesniak, L. and B. Loiseau, 
{\em S-, P- and D-wave $\pi\pi$ final state interactions and CP violation in $B\pm \to \pi\pm\pi\mp\pi\pm$ decays },
Acta Phys. Polon. {\bf B42}, 2013 (2011); arXiv:1011.0960.
 
\vskip .2cm
\bibitem{BD} G. Burdman and J.F. Donoghue, 
{\em Union of chiral and heavy quark symmetries},
Phys. Lett. B {\bf 280}, 287 (1992).

\vskip .2cm
\bibitem{wise} M.B. Wise, 
{\em Chiral perturbation theory for hadrons containing a heavy quark},
Phys.Rev. D{\bf 45}, R2188 (1992).

\vskip .2cm
\bibitem{GL} J. Gasser and H. Leutwyler,
{\em Chiral Perturbation Theory: Expansions in the mass of the strange quark},
Nucl. Phys. B{\bf 250}, 465 (1985);
{\em Chiral perturbation theory to one loop},
Ann. Phys. {\bf 158}, 142 (1984).

\vskip .2cm
\bibitem{EGPR} G. Ecker, J. Gasser, A. Pich and E. De Rafael,
{\em The role of resonances in  Chiral Pertubation  Theory},
Nucl. Phys. B {\bf 321}, 311 (1989).

\vskip .2cm
\bibitem{Bernard}
 V. Bernard, N. Kaiser and U.G. Meissner, 
{\em $\pi K$ scattering in chiral perturbation theory to one loop},
Nucl. Phys. B {\bf 357}, 129 (1991).

\vskip .2cm
\bibitem{CGL} G. Colangelo, J. Gasser and H. Leutwyler,
{\em $\pi\pi$ scattering },
Nucl. Phys. {\bf B603}, 125 (2001).

\vskip .2cm
\bibitem{Pelaez} R. Kaminski, J. R. Pelaez, F. J. Yndurain, 
{\em Pion-pion scattering amplitude. II. Improved analysis above $\bar{K}K$ threshold},
Phys. Rev. D {\bf 74}, 014001 (2006); Erratum-ibid. D 74, 079903 (2006). 

\vskip .2cm
\bibitem{Moussalam}
P. B\"uttiker, S. Descotes-Genon and B. Moussalam,
{\em A new analysis of $\pi K$ scattering from Roy and Steiner type equations},
Eur. J. Phys. C {\bf 33}, 409 (2004).

\vskip .2cm
\bibitem{lc09} K.S.F.F. Guimar\~aes, W. de Paula, I. Bediaga,
A. Delfino, T. Frederico, A. C. dos Reis
and L. Tomio, {\em hree-body model of the final state interaction in heavy meson decay},
Nucl. Phys. B (Proc. Suppl.) \textbf{199}, 341 (2010).

\vskip .2cm
\bibitem{Diogo} D.R. Boito and M.R. Robilotta,
 {\em Scalar resonances: Scattering and production amplitudes}
Phys. Rev. D {\bf 76}, 094011 (2007).

\vskip .2cm
\bibitem{PatThesis} P.C. Magalh\~aes, Ph.D. Thesis, 
University of S\~ao Paulo (2014). 

\vskip .2cm
\bibitem{GS}  G.J. Gounaris and J.J. Sakurai, 
{\em Finite-width corrections to the vector-meson-dominance prediction for $\rho \to e^+ e^-$}
Phys. Rev. Lett. {\bf 21}, 244 (1968).


% Patricia's and Mane'a references
\vskip .2cm
\bibitem{BW} G. Breit and E. Wigner, 
{\em Capture of slow neutrons}
Phys. Rev. {\bf 49}, 519 (1936).

\vskip .2cm
\bibitem{BD}  Bjorken and Drell, {\em Relativistic Quantum Mechanics},  New York, McGraw-Hill (1964).

\vskip .2cm
\bibitem{Scherer}  S. Scherer, 
{\em Introduction  to Chiral Pertubation Theory}, 
Adv. Nucl. Phys. {\bf B622}, 207 (2005); hep-ph/0504116. 

\vskip .2cm
\bibitem{LSB}  L.S. Brown, {\em Quantum Field Theory},   
Cambridge University Press. (1994).

\vskip .2cm
\bibitem{OO} J.A. Oller and E. Oset, 
{\em N/D description of two meson amplitudes and chiral symmetry}
Phys. Rev. D {\bf 60}, 074023 (1999);
see also Ref. [74].

\end{thebibliography}





==> lhcb-v2-copy.tex <==
%\documentclass[superscriptaddress,a4paper,9pt,aps,amsfonts,amsmath,nofootinbib,byrevtex,prd,preprint,twocolumn]{revtex4-1}   
%\documentclass[aps,prd,nofootinbib,twocolumn,superscriptaddress,showpacs,preprintnumbers]{revtex4-1}
% \usepackage{epsfig,dcolumn}
% \usepackage{graphicx}
% \usepackage{color}

% \usepackage{amsmath}
% \usepackage{amsfonts}
% \usepackage{amssymb}
% \usepackage{graphicx}
% \usepackage{bm} % scaled bold math symbols

 
% \newcommand{\be}{\begin{equation}}
% \newcommand{\ee}{\end{equation}}

% \DeclareMathOperator{\re}{Re}
% \DeclareMathOperator{\im}{Im}


% %%%%%%%%%%  END OF PREAMBLE  %%%%%%%%%%

% \begin{document}

\title{Analytical improvements to Breit-Wigner isobar models} 

%\author{V. Mathieu$^{1,2}$, G. Fox$^{3}$  and A. P. Szczepaniak$^{1,2,4}$} 
%\affiliation{
% $^1$ Department of Physics, Indiana University, Bloomington, IN 47405, USA \\
% $^2$  Center for Exploration of Energy and Matter, Indiana University, Bloomington, IN 47403, USA\\
% $^3$ School of Informatics and Computing, Indiana University, Bloomington, IN 47405, USA \\
 %$^4$  Jefferson Laboratory, 12000 Jefferson Avenue, Newport News, VA 23606, USA } 


\author{Adam~P.~Szczepaniak}
\affiliation{Center for Exploration of Energy and Matter, Indiana University, Bloomington, IN 47403}
\affiliation{Physics Department, Indiana University, Bloomington, IN 47405, USA}
\affiliation{Thomas Jefferson National Accelerator Facility, %12000 Jefferson Avenue,  
Newport News, VA 23606, USA}


\begin{abstract}
We discuss the derivation and properties of the general representation of partial wave amplitudes in the context of improving the models currently used in analysis of three particle Dalitz distributions. 
\end{abstract}

%\pacs{11.55.Fv, 11.55.Hx, 12.40.Nn, 13.75.Gx}

\maketitle

\section{introduction}
In this note, after a brief introduction to aspects of  $S$-matrix theory 
 relevant in the analysis of three particle Dalitz plots, I focus on properties of Breit-Wigner (BW) amplitudes and the isobar model in general.  I discuss the LHCb analysis model in the context of 
 a general  isobar-type approximation and  show, for example, 
   which features of the  BW amplitude, {\it e.g.} barrier factors,  Blatt-Weisskopf factors, {\it etc.} are universal    and which are not,  {\it i.e.}  are process dependent.  The possibility of extending the BW description in a way that is consistent with analyticity, unitarity, and even crossing 
    would allow to access systematic uncertainties in data analysis. I concentrate on spinless particles. 
     Spin introduces kinematical complexities but  
    does not affect how unitarity, analyticity, and crossing are implemented, at least for a finite set of partial waves. 

 \section{Kinematical vs Dynamical Singularities} 
 
 We are interested in amplitudes describing a decay of a  quasi-stable particle $D$ with mass $M$ to 
  three  distinguishable particles  $A,B,C$  
  
\begin{equation} 
D  \to A + B + C   \label{D} 
\end{equation} 
 The decay amplitude depends on particle helicities,  $\lambda_i$, 
 $i=A,B,C,D$,   and  three Mandelstam invariants, which we define as $s = (p_A + p_B)^2$, $t = (p_B + p_C)^2$ and $u=(p_A + p_C)^2$. The invariants  are kinematically constrained by $s + t + u = \sum_i m_i^2$.  Analytical $S$-matrix theory states that, besides the decay channel, the same amplitude describes each of the three  two-to-two scattering process, {\it i.e} the $s$-channel reaction $D + \overline{C} \to A + B$, (bar denotes an antiparticle) as well as the $t$ and $u$ channel scattering.  What this means in practice is the following. For each combination of helicities  there is an analytical function $A_{\lambda_i}(s,t,u)$ of the three complex Mandelstam variables and complex $M^2$, such that the three physical 
    scattering amplitudes and the decay channel amplitude correspond to the limit of $A_{\lambda_i}$ 
     when  $s,t,u,$ and $M$ approach the real axis in the physical domain of the corresponding  reaction. 
 This is the essence of crossing symmetry. 
 In general crossing mixes helicity amplitudes and leads  
  to complicated relations for helicity amplitudes. Furthermore,  
     helicity amplitudes have kinematical singularities in the Mandelstam variables. 
% I don't understand this sentence: These are enforced by absence of such singularities in a covariant 
%representation.
 Despite such complexities it is possible to come up with parameterizations of helicity amplitudes that take into account both  kinematical and dynamical constraints~\cite{MartinSpearman}. 
   On the other hand it is also useful to consider 
    the  covariant from  {\it i.e.} a representation of helicity amplitudes in terms of  Lorentz-Dirac factors 
 that describe wave functions of the free particles participating in the reaction. The advantage of the covariant representation is that the scalar functions multiplying all independent covariants are simply related by crossing and are free from kinematical singularities. At the end of the day one still needs the 
     helicity amplitudes for partial wave analysis. In ~\cite{Danilkin:2014cra} the reaction $\omega \to \pi^+\pi^-\pi^0$ was  studied and this example provides a good illustration of the issues discussed above. 
         

The main postulate of relativistic reaction theory is that reaction amplitudes are analytical functions of kinematical variables. It follows from Cauchy's theorem  that an analytical function is fully determined by its domain of analyticity, {\it i.e.} location of singularities. Thus knowing amplitude singularities allows 
to determine the amplitude elsewhere, including the various physical regions. 
     In S-matrix theory it is assumed that all singularities 
   can be traced to unitarity. In the absence of an explicit solution to the scattering problem in QCD, 
   analyticity and unitarity  provide the least model dependent description  of hadron scattering. 
    
  Unitarity operates in any of the Mandelstam variables. 
 In the  $s$-channel the physical domain is located on the positive real axis in the $s$-plane above the elastic threshold.    Unitarity makes amplitudes singular at each open channel threshold, the singularity being of the square-root type. The same happens in variables $u$ and $t$.  The amplitude  also has singularities in the variable $M$ since it represents an unstable channel. In studying a particular decay process, {\it e.g.} $J/\psi \to 3\pi$,  $M$ is fixed in a very narrow range (within the width of the $J/\psi$),  and dependence on $M$ is effectively fixed and its singularity structure irrelevant. 
   
 
In general,  it is not known how to write an amplitude that has correct unitarity 
 constraints in two or more overlapping channels. The reason being that it is only simple to implement 
  unitarity on partial waves where it is an algebraic constraint. A single partial wave in one channel corresponds to an infinite number of partial  waves in another one thus imposing unitarity on say both $s$ and $t$-channel partial waves simultaneously requires an infinite number of partial waves. Regge theory  extends the 
  concept of analytical continuation to the angular momentum variable of partial waves. Singularities in the angular  momentum plane  {\it e.g.} Regge poles, determine the behavior of infinite sums of partial waves, thus Regge theory is used to implement  cross channel unitarity. 
 
 
 In general, amplitude singularities are known only in a limited domain, but as long as they dominate in 
  a kinematical region of interest one may be able to construct a realistic amplitude model.  Amplitude models fall into two main categories. One is that of dual models, {\it e.g.} the Veneziano model and  the other is the isobar  model category,  {\it e.g.} the Khuri-Treiman model. Dual models attempt to incorporate $S$-matrix constraints directly on the full amplitude that depends on the Mandelstam variables. 
  Since isobar is synonymous with a partial wave, isobar models are models based on a (truncated) partial wave expansion. 

   In the following I will discus the isobar model in some detail since this is almost exclusively the model used at present in analyses of three particle Dalitz distributions. 
 
  
 \section{The Breit-Wigner amplitude} 
 
 In the  Breit-Wigner formula, a partial wave, $f_l(s)$ is approximated by a pole in $s$ 
  located in the complex energy plane at $s_P = Re s_P - i \mathit{Im} s_P$, 
\begin{equation} 
f^{p}_l(s) \propto \frac{1}{s_P - s}  \label{p} 
\end{equation} 
 The real and imaginary parts are related to the mass,  $M = \sqrt{Re\, s_P}$  and the width, $\Gamma = Im\, s_P/M$  of a resonance. For comparison with experiment a reaction amplitude 
  is evaluated at physical, real values of  kinematical variables {\it e.g} when $s$ approaches
    the real axis from above. The contribution form a  BW  pole to a partial cross section, $\sigma_l$ is  proportional to 

\begin{equation} 
\sigma_l \propto \lim_{\epsilon \to 0} |f^p_l(s + i\epsilon) |^2 \propto \frac{1}{(s - M^2)^2 + (M \Gamma)^2}.  
\end{equation} 

Since the resonance pole is located in the complex s-plane, on the real s-axis,  where experimental data is taken, it produces a smooth variation in the cross section. The closer the pole is to  the real axis, {\it i.e.} the smaller the resonances width, the more rapid is the variation in cross section or event distribution. 
It is worth keeping in mind that once energy  is considered as a complex variable any variation of the reaction amplitude in the physical region can be traced to the existence of singularities in the complex energy plane 
  {\it e.g.} a pole as in the BW formula.   


   \section{ Unitarity and the Breit-Wigner amplitude} 
   
 The BW formula of Eq.~(\ref{p}) is an analytical function of $s$ except for a single pole at $s=s_P$. How does unitarity constrain the BW pole? Resonance decay is possible because of open channels and it is unitarity that controls the distribution of probability across decays.  It thus follows that unitarity must 
  constrain resonance decay widths and thus the imaginary part of the BW pole. But Eq.~(\ref{p})  is only an approximation to the ``true", unitary amplitude valid for $s$ near the position of the complex pole. 
 Since  unitarity operates in the physical domain, {\it i.e.} 
       on the real axis, the constraint of unitarity on the ``true" amplitude is lost in the pole approximation, {\it i.e.} at a finite distance from the real axis. In this case implementing unitarity is related to using 
       energy dependent widths. 

      Suppose the lowest mass open channel is a state of  particles $A$ and $B$ with threshold at $s=s_{th} = (m_A + m_B)^2$. In the mass range between $s_{th}$  and the first threshold, 
    unitarity constrains the ``true" amplitude to satisfy
   
   \begin{equation} 
   Im \hat f_l(s) = \hat t^*_l(s) \rho_l(s) \hat f_l(s).  \label{f} 
  \end{equation} 
  Here $\hat f_l(s)  =  f_l(s)/(a q)^{l}$  and $\hat t_l(s) = t_l(s)/(a q)^{2l}$ are the $s$-channel 
   reduced partial waves 
    representing production  of $AB$ in $D + \overline{C} \to A + B$ and elastic $A + B \to A + B$ scattering, respectively. Near threshold $q\to0$, with  $q$  being the relative momentum between $A$ and $B$ in the 
     $s$-channel center of mass frame,  partial waves vanish as $(aq)^l$,  where $a$ is given 
      by the position of the lowest mass singularity in the crossed channels, {\it i.e.} the range of interaction.  $\rho_l(s)$ is a known kinematical function describing the two-body phase space. It has 
      a  square-root  branch point at $s = s_{tr}$. As $s$ increases beyond the first inelastic threshold, $Im \hat f_l(s)$ receives a  ``kick" from another square-root type singularity form channel openings  
       and the {\it r.h.s} of Eq.~(\ref{f}) needs to be modified.  Eventually three and more particle channels open. 
        In practice unitarity is a useful constraint in a limited energy range that covers a small number of open channels  {\it e.g.} close to the elastic threshold. 
              Replacing, in Eq.~(\ref{f}),  $\hat f_l$  by $\hat t$ one obtains the unitarity relation for the elastic 
         $A + B \to A + B$ partial waves in the elastic region, 
   \begin{equation} 
   Im \hat t_l(s) = |\hat t(s)|^2 \rho_l(s). \label{t} 
  \end{equation} 
 Above the inelastic threshold the {\it r.h.s} of Eq.~(\ref{t}) should be modified as discussed above. 
  In case there is a finite number $N$  of  relevant inelastic channels, the unitarity condition can be expressed in a matrix form 
\begin{equation} 
Im \hat t_{l,ij}(s) = \sum_k  \hat t_{l,ik}^*(s) \rho_{l,k}(s) \hat t_{kj}(s) 
\end{equation} 
 where $\hat t_{l,ij}(s) = t_l(s)/(aq)^{l_i}(aq)^{l_j}$  and 
 $\rho_{l,k}(s)$ is the appropriate, reduced phase space in channel $k$. 
 The unitarity relation for $\hat f_{l,i}(s)$ takes on a similar form, 
\begin{equation} 
Im \hat f_{l,i}(s) = \sum_k  \hat t_{l,ik}^*(s) \rho_{l,k}(s) \hat f_{k}(s). 
\end{equation} 

For a given $\hat t_l(s)$,  the analytical amplitude $\hat f_l(s)$ that satisfies Eq.~(\ref{f}) can be written as  

    \begin{equation} 
  \hat f_l(s) = \hat t_l(s) G_l(s)  \label{sf} 
  \end{equation} 
and sometimes the so-called Muskhelishvili-Omnes function is used instead of $\hat t_l(s)$ on the {\it r.h.s} of Eq.~(\ref{sf})   \cite{Pham:1976yi}.  The function $G_l(s)$ is an analytical function of $s$ with cuts 
 except on the real axis in the elastic region. The latter are accounted for by the elastic amplitude $t_l(s)$. 
  The singularities  of $G_l(s)$ correspond to the (often unknown) contributions from the unitarity-imposed 
   left hand cuts cuts that exist in the crossed, $t$ and $u$ channels. 
 The inelastic contributions {\it i.e.}  right cuts in $\hat f_l$ are related to the inelastic contributions to the amplitude    $\hat t_l(s)$ which is easy to show if the matrix representation is used, 
   \begin{equation} 
   \hat f_{l,i} = \sum_k \hat t_{l,ik} G_{l,k}(s) \label{sf2}
   \end{equation} 
 and with the functions $G_{l,k}(s)$ bearing only left hand cuts.    
     Now we go  back to the pole formula. From Eq.~(\ref{f})  it follows that poles of the production amplitude  
     $\hat f_l$ are also poles of $\hat t_l$. This is because no resonance poles appear on sheets connected 
   to the left hand cuts~\cite{gribov}.  Since $\hat t_l(s) $  satisfies  Eq.~(\ref{t}) it can be shown that the most general parametrization has the form, 
  \begin{equation} 
  t_l(s) = \frac{1 }{ C_l(s)  - I_l(s)  } \label{st} 
  \end{equation}
  which in the inelastic case generalizes to the matrix form 
  \begin{equation} 
  t_{l,ij}(s) = [ C_{l}(s) - I_l(s) ]^{-1}_{ij} 
  \end{equation}
 with $C_l$ and $I_l$ becoming   $N\times N$ matrices in the channel space.   
     The function $C_l(s)$ ($C_{l,ij}(s)$)   has  similar properties to the function $G_l(s)$  ($G_{l,i}(s)$)  in Eq.~(\ref{sf}),     {\it i.e.} it is real for real $s$ in the elastic region and have only left hand cuts. 
   The function $I_l(s)$ is a known analytical function {\it i.e.} the Chew-Mandelstam function, 
  %given by 
%\begin{equation}  
 %I(s) =   \frac{s}{\pi} \int ds' \frac{\rho(s')}{s' (s' - s)} 
 %\end{equation} 
with its imaginary part for real $s$ given by $Im I_l(s) = \rho_l(s)$. 
The reason why the analytical solution of Eq.~(\ref{t}) is more complicated than that of Eq.~(\ref{f}), is that the former is a non-linear relation for the amplitude. It is easy to check that this equation becomes a linear condition for the inverse of $\hat t_l$  
 and this is the reason why dependence on phase space appears in the denominator in Eq.~(\ref{st}). 
 It is straightforward  to check that Eq.~(\ref{st}) satisfies Eq.~(\ref{f}), or in the inelastic case,  its matrix generalization.  The presence of  ``denominators" in amplitudes are a direct consequence of unitarity and so are the resonance  poles, which correspond to zeros of the denominators. 
  
  
  One  immediately recognizes that the $K$-matrix, or the $K$ function in the elastic case,  
   corresponds to 
 \begin{equation} 
 K^{-1}_l(s) = C_l(s) - Re I_l(s). 
 \end{equation} 
 Since the real  part of a function is not an analytical function, an analytical approximation to the $K$ matrix 
  violates analyticity of the amplitude and may lead to spurious ``kinks" from square-root unitarity branch points in the physical region. 
 It  is much better to use Eq.~(\ref{st}), {\it aka} the Chew-Mandelstam representation, with the analytical ($K$-matrix type) parametrization reserved for the analytical  function $C_l(s)$. 
       
  Combining Eq.~(\ref{st}) with Eq.~(\ref{sf}) one obtains 
  \begin{equation} 
  \hat f_l(s) = \frac{G_l(s)}{C_l(s) - I_l(s)}  \label{solf1} 
  \end{equation} 
  or in the matrix form for the inelastic case 
  \begin{equation} 
  \hat f_{l,i}(s) = \sum_k [C_l(s) - I_l(s)]^{-1}_{i,k} G_{l,k}.  \label{solf2} 
  \end{equation} 
  
  
  Now we can finally see how  the BW  pole formula of Eq.~(\ref{p})  emerges. Suppose in Eq.~(\ref{solf1}) the denominator vanishes  at some complex $s= s_p$. Near the pole  of  $\hat f_l$ 

\begin{equation} 
 \hat  f_l(s) \sim \frac{\beta_l}{s - s_p}  
  \end{equation} 
  where 
  \begin{equation} 
  \beta_l = G_l(s_p)/(C'_l(s_p) - I'_l(s_p)).
  \end{equation} 
  In the inelastic case the role of the denominator in the {\it r.h.s} of  Eq.~(\ref{solf1}) is  played by the  determinant of the $N \times N$ matrix $[C_l(s) - I_l(s)]$. 
  Even though the residue of the pole $\beta_l$  is in general  a complex number, it can be shown that only its magnitude is to be related with  a coupling of a resonance to a decay channel~\cite{gribov}. The residue $\beta_l$ should be distinguished from the numerator $G_l(s)$. The latter is energy dependent and represents the production amplitude of the final state  $A + B$ given the initial state $D + \overline{C}$. The former is a number representing the  product of couplings of the resonance to the  initial and final states. 
     
 Finally we  ``derive" the more familiar  BW formula, with energy dependent widths. In  the ``LHCb" notation 
 \begin{equation} 
 f^{LHCb}_{l_s}(s) = F_{l_s}(q) R_{l_s}(s) F_{l_t}(p)  
 \end{equation} 
 so that the reduced amplitude is given by 
 \begin{equation} 
 \hat f^{LHCb}_{l_s}(s) = \frac{ F_{l_s}(q)}{(aq)^{l_s}} R_{l_s}(s) F_{l_t}(p)
 \end{equation} 
 where $q = q(s)$ is the decay channel relative momentum between $A$ and $B$ 
  and $p = p(s)$ is the decay channel relative momentum between the $(AB)$ pair and the spectator particle $C$. For comparison with the analysis given above all that is needed is to replace the decay channel expressions for $q$ and $p$ by the $s$-channel ones. 
 The function $F_l(x)$ is a product of an angular momentum barrier factor  $x^{l}$ and a Blatt-Weisskopf  factor   
 \begin{equation} 
 F_l(x) = (ax)^l F'_l(x)
 \end{equation} 
where, for example, 
 \begin{equation} 
 F'_2(q) =  \sqrt{\frac{13}{((aq)-3)^2 + 9(aq)}}  
 \end{equation} 
 The propagator $R_{l_s}(s)$ is given by 
 \begin{eqnarray} 
& &  R_{l_s}(s) = \frac{1}{ m_r^2 - s - i \rho_{l_s}(s) X(p) } \nonumber \\
 & &  = 
  \frac{1}{  X(p) (  C^{LHCb}(s) -  i \rho_{l_s}(s) ) }, \, C^{LHCb}(s)   \equiv \frac{m_r^2 - s}{X(p)}  \nonumber \\
 \end{eqnarray} 
 so that one can rewrite the LHCb amplitude model as 
 \begin{equation} 
 \hat f^{LHCb}_{l_s}(s) = \frac{G^{LHCb}_{l_s}(s)}{ C^{LHcB}(s) - i\rho_{l_s}(s) }  \label{BWlhcb} 
 \end{equation} 
 where 
 \begin{equation} 
 G^{LHCb}_{l_s}(s)   =  \frac{F'_{l_s}(q) F_{l_t}(p)}{X(s)}. 
 \end{equation} 
 Eq.~(\ref{BWlhcb}) is a specific case of Eq.~(\ref{solf1}). It is in fact the $K$ matrix (function) approximation 
 since only the imaginary part, $\rho_{l_s}(s)$ of the dispersive integral $I_l(s)$ is used.
   The functions $C_l$ and $G_l$ containing, through left hand cuts,  physics of elastic production of $AB$ in  $A + B \to A + B$ and  in decay $D  \to A + B + C$, respectively, 
    have been replaced by a specific product of Blatt-Wisskopf factors. The latter originate 
     from a potential model in non-relativistic scattering and at best can be considered as a crude  approximation. In precision data analysis they should be replaced by a more flexible 
       parametrization.  In LHCb, analysis contributions from several poles are included by adding 
        BW amplitudes. Eq.~(\ref{solf1}) shows how all such poles need to appear as zeros of the common denominator. Finally the matrix representation of Eq.~(\ref{solf2})  is  the correct formula for dealing with multiple channels. 
   
   
   
   \section{ Combining $s$, $t$, and $u$, channel isobars and corrections to the isobar model} 
 
In the previous section we discussed  how the energy dependent  BW amplitude is related to the general 
 expression for the partial wave. Here we discuss how the partial wave amplitudes build the full amplitude in the decay channel. 
 
In the scattering domain of the $s$-channel, the  partial wave expansion of the full amplitude 
 converges and a finite number of partial waves waves may give a good approximation to the whole sum.  Energy dependence of individual 
  partial waves can be represented using expressions like the one in Eq.~(\ref{sf}) or  Eq.~(\ref{sf2}). 
  In a decay channel, the partial wave series also  converges, but one cannot simply replace the one sum but the other. This is because  the decay channel partial waves have extra ''complexity'' compared to the scattering channel, due to $t$ and $u$ channel singularities, {\it i.e.} resonances begin in the physical region. 
     Ignoring spins of external particles,    the $s$-channel partial wave series is given by 
  \begin{equation} 
  A(s,t,u) = \frac{1}{4\pi} \sum_{l=0}^\infty (2l+1) f_l(s) P_l(z_s). \label{spw} 
  \end{equation} 
On the {\it r.h.s} the dependence on $t$ and $u$ is algebraic, through $z_s$ and the rotational functions. Thus in the physical domain of the decay,  the $s$-channel series diverges because the {\it l.h.s} has singularities in $t$ and $u$. Furthermore, it follows that any truncated, finite set of $s$-channel partial waves cannot reproduce $t$ or $u$-channel singularities, {\it e.g.} resonance which appear inside the Dalitz plot. These issues are resolved in the isobar model by replacing the infinite number of $s$-channel partial waves by a  finite set and  adding  a (finite)  set of $t$ and $u$ channel partial waves. Thus the amplitude has a mixed form that includes partial waves (isobars) in the three channels simultaneously, 
 
 \begin{equation}
 A(s,t,u) = \frac{1}{4\pi} \sum_{l=0}^{L_{max}} (2l+1) a^{(s)}_l(s) P_l(z_s)  + (s \to t) + (s \to u) \label{im} 
 \end{equation} 
 We refer to $a^{(s)}_l(s)$ as the isobaric amplitude in the $s$-channel and analogously, 
   $a^{(t)}_l(t)$ and $a^{(u)}_l(u)$ are the isobaric amplitudes in the $t$ and $u$-channels, respectively. 
 In a typical Dalitz plot analysis, the isobaric amplitudes are parametrized using the energy dependent BW amplitudes discussed in the previous sections.  
 
 Projecting the {\it r.h.s} of Eq.~(\ref{im}) into the $s$-channel gives the $s$-channel partial waves, which 
   we denoted by $f_l(s)$,  
 \begin{eqnarray} 
& &  f_l(s)  = a^{(s)}_l(s) \nonumber \\
& &  +\frac{1}{2} \int_{-1}^1  dz_s P_l(z_s) \sum_{l'=0}^{L_{max}} (2l' + 1) a^{(t)}_{l'}(t) P_{l'}(z_t) + (t \to u) \nonumber \\  & & \equiv a^{(s)}_l(s) + b^{(s)}_l(s). 
 \end{eqnarray} 
 Under the integral, $t$ and $u$ are to be considered as function of $s$ and $z_s$, the cosine of the $s$-channel scattering angle.  Since the integral contributes to partial waves with arbitrary $l$, Eq.~(\ref{im}) defines a model   for an infinite number of partial waves $f_l(s)$ and gives the result of the  analytical continuation of the   series in Eq.~(\ref{spw}).  
Application of unitarity in the $s$-channel leads to a relation between the isobaric  amplitudes 
\begin{equation} 
a^{(s)}_l(s) = t_l(s) \left[ \frac{1}{\pi} \int_{s_{tr}} ds' \frac{ \rho_l(s') b^{(s)}_l(s')}{s' - s} \right]. \label{a} 
\end{equation} 
The amplitude  $b^{(s)}_l(s)$ is  the $s$-channel projection of the $t$ and $u$ channel exchanges. 
 As a function of $s$ it has a left hand cut but no right hand, unitary  cut. The 
dispersive integral in Eq.~(\ref{a})  has the $s$-channel unitary cut. 
 Thus $s$-channel unitarity demands that the $s$-channel isobaric amplitude $a^{(s)}_l(s)$ has the right cut 
  coming not only form the elastic $A + B \to A + B$ amplitude, $t_l(s)$, but also from the dispersion of $s$-channel projections of the  $t$ and $u$-channel amplitudes. It is important to note this difference between the partial wave amplitudes $f_l(s)$ and the isobaric amplitudes $a^{(s)}_l(s)$. In case of the former the right hand cut discontinuity comes entirely  from the elastic scattering, {\it c.f.} Eq.~(\ref{sf}),~(\ref{sf2}). In the isobar model, the partial wave amplitudes are given by, 
\begin{eqnarray}  
& &  f_l(s) = t_l(s) \left[ \frac{ b^{(s)}_l(s) }{t_l(s)}+  \frac{1}{\pi} \int_{s_{tr}} ds' \frac{ \rho(s') b^{(s)}_l(s')}{s' - s} \right]  \nonumber \\
& & \equiv  t_l(s) G_l(s)  
\end{eqnarray} 
which are indeed of the form given by Eq.~(\ref{sf}), since it can be shown that the right hand cuts cancel between the two terms in the square bracket so that  $G_l(s)$ has only left hand cuts, 


\begin{equation}  
  G_l(s) =  \frac{1}{\pi} \int_{s_{tr}} ds' \rho(s') \frac{  b^{(s)}_l(s') - b^{(s)}_l(s)}{s' - s}.
\end{equation} 


 In the inelastic case this generalizes to the form given by Eq.~(\ref{sf2}). 
 The left hand cuts, as expected, originate from exchanges in the crossed channels determined by the amplitude $b^{(s)}_l(s)$. 
  
   One goes further and also  impose $t$ and $u$-channel unitarity, thereby correlating isobar expansions in the three channels. This is the analytical, unitary description of ``final state interaction"   that relies on the model independent features of the amplitudes only. 
 
  The implications for event distributions  in the Dalitz plot, given the left hand cut singularities of 
  $b^{(s)}_l(s)$,  were studied in ~\cite{schmid}. In the next section we take a  look at the left hand cuts of the amplitude $G_l(s)$. 

  
       


  \section{Watson's theorem} 
  Since the imaginary part of a complex function is itself a real function, it follows from Eq.~(\ref{f}) that in the elastic region, the phase of $\hat f_l(s)$ equals that of the elastic scattering amplitude $\hat t_l(s)$. 
It is often forgotten to be mentioned, however, that in many cases the {\it r.h.s}  in 
 Eq.~(\ref{f}) does not saturate the imaginary part even in the elastic regime. When this happens,  Watson theorem is violated even in the elastic regime. And this is the case for a decay process. In this case there is nevertheless a relation between $\hat f_l$ and $\hat t_l$, or a generalized Watson relation. 
 
 In the decay kinematics, even if  the energy of the $A B$ state is below the inelastic threshold, the imaginary part of the $s$-channel partial amplitude, $\hat f_l(s)$,   is not in given by Eq.~(\ref{f}). 
  In this case because  in the decay kinematics,  cross channel singularities (from thresholds/unitarity) {\it e.g.} isobar exchanges in $t$ or $u$ channel,  are located in the physical region of the $s$-channel and contribute to the imaginary part of the  $s$-channel partial wave. Another way of saying this, is that in the decay kinematics singularities of $\hat f_l(s)$, which otherwise are to the left of the  elastic unitarity cut,  move to the right of the elastic unitary branch point.  
 
In the previous section we argued that  Eq.~(\ref{sf}) follows from the assumption that $\hat f_l(s)$ is an analytical function.  The relation between analyticity and casualty applies to full amplitudes, while partial waves are related to full amplitudes in a complicated way. Analytical partial waves are  obtained by a continuation of the unitary relation to the complex energy plane. It can be shown  (see {\it e.g.} \cite{gribov}) 
  that when left and right hand cuts are separated $Im \hat f_(s)   = \Delta \hat f(s_+) \equiv  (\hat f_l(s_+) - \hat f_l(s_-) )/2i $, where $s_\pm = s \pm  i \epsilon $. That is,  the imaginary part of the amplitude as measured in the experiment, which by itself is a real function, is  equal to the discontinuity across the real axis of the unique extension of $\hat f_l(s)$ to the complex energy plane. It turns out,  however,  that in decay kinematics, the proper extension of $\hat f_l(s)$ to the complex energy plane is such that in 
  Eq.~(\ref{f}) the {\it l.h.s} should be replaced by 
 $\Delta f(s_+)$ and the {\it r.h.s} should be replaced by the product 
 $t_l(s_-) \rho_l(s) f_(s_+)$.  Thus, elastic unitarity still determines the discontinuity across the right hand cut but it is no longer a real function. This is the generalized Watson or discontinuity relation. 


 As a result the representation given by Eqs.~(\ref{sf}),(\ref{sf2}) is still valid 
with  the exception that the numerators, $G_l(s)$ become complex in the elastic region. They do not have the unitarity cut though. Just like in the ``standard" Watson's theorem the right hand cut discontinuity comes entirely from the elastic amplitude $t_l(s)$.  The  complexity of $G_l(s)$ is still of the left hand cut nature, except that left hand cuts have moved onto the right hand side under the right hand cut and into the second sheet. 
\cite{Szczepaniak:2015eza}. 
 
 
\section*{Acknowledgments}
I would like to thank the organizers and participants of the LHCb workshop on multi-body decays of B and D mesons for stimulating discussions. 
 This  work is  supported by the U.S. Department of Energy, Office of Science, Office of Nuclear Physics under contract DE-AC05-06OR23177. It is  also supported in part by the U.S. Department of Energy under Grant No. DE-FG0287ER40365.




% \begin{thebibliography}{40}

% \bibitem{MartinSpearman} 
% A.D. Martin and T.D. Spearman, {\it Elementary Particle Theory}, (North-Holland, Amsterdam, and Elsevier, New York, 1970.) 

% \bibitem{Danilkin:2014cra} 
%   I.~V.~Danilkin, C.~Fern·ndez-RamÌrez, P.~Guo, V.~Mathieu, D.~Schott, M.~Shi and A.~P.~Szczepaniak,
%   %``Dispersive analysis of ?/??3?,??*,''
%   Phys.\ Rev.\ D {\bf 91}, no. 9, 094029 (2015)
%   [arXiv:1409.7708 [hep-ph]].
  
%  \bibitem{Pham:1976yi} 
%   T.~N.~Pham and T.~N.~Truong,
%   %``Muskhelishvili-Omnes Integral Equation with Inelastic Unitarity: Single and Coupled Channel Equations,''
%   Phys.\ Rev.\ D {\bf 16}, 896 (1977).
%   %%CITATION = PHRVA,D16,896;%%
 
%  \bibitem{gribov} 
% V.N.~Gribov, J.~Nyiri, Y.~Dokshitzer, {\it  Strong interactions of hadrons at high energies : Gribov lectures on theoretical physics}, (Cambridge University Press Cambridge, UK, New York 2009). 


% \bibitem{Szczepaniak:2015eza} 
%   A.~P.~Szczepaniak,
%   %``Triangle Singularities and XYZ Quarkonium Peaks,''
%   Phys.\ Lett.\ B {\bf 747}, 410 (2015)
%   [arXiv:1501.01691 [hep-ph]].
 
 
%  \bibitem{schmid} 
%  C.Schmid, Phys. Rev. 154, 1363 (1964). 
% \end{thebibliography}

  
%   \end{document} 


